X-ray Hotspots in the Northwest Shell of the Supernova Remnant RX J1713.7$-$3946

The supernova remnant (SNR) RX J1713.7$-$3946 is one of the best-studied accelerators of cosmic rays because of its strong nonthermal X-ray and gamma-ray radiation. We have analyzed accumulated \chandra\ observations with a total exposure time of $\sim$266 ks in the northwest rim of RX J1713.7$-$3946. We detect a substantially large number of point-like sources, referred to as ``hotspots'', which are likely associated with the remnant. The spectra of the hotspots are well described by an absorbed power-law model. The spectral properties ($10^{21}\ \mathrm{cm^{-2}}\lesssim N_H \lesssim 10^{23}\ \mathrm{cm^{-2}}$ and $ 0.5\lesssim \Gamma \lesssim 6$) are different from diffuse X-ray emission in RX J1713.7$-$3946, and the harder hotspot tends to have the larger $N_H$. We also confirm yearly and monthly variabilities of flux for some hotspots. We propose that RX J1713.7$-$3946 is embedded in a complex surroundings where some dense molecular clumps and cores exist inside a wind-blown cavity, and that the hotspot traces synchrotron emission caused by an interaction of shock waves of the SNR and dense molecular cores with a number density of $10^{5}-10^{7}~ \mathrm{cm}^{-3}$. The X-ray radiation of the hotspot might be emitted from both primary electrons accelerated at the shocks and secondary electrons produced by the interaction of accelerated protons with the cores.

==> higurashi_hot-spot_abst.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% abstract

A supernova remnant (SNR) \rxj\ is one of the best-studied accelerators of cosmic rays because of its strong nonthermal X-ray and gamma-ray radiation.
We have analyzed accumulated \chandra\ observations with a total exposure time of $\sim$266 ks in the northwest rim of \rxj.
We detect a substantially large number of point-like sources, referred to as ``\hsS'', which are likely associated with the remnant.
The spectra of the \hsS\ are well described by an absorbed power-law model.
The spectral properties ($10^{21}\ \mathrm{cm^{-2}}\lesssim N_H \lesssim 10^{23}\ \mathrm{cm^{-2}}$ and $ 0.5\lesssim \Gamma \lesssim 6$) are different from diffuse X-ray emission in \rxj, and the harder \hs\ tends to have the larger $N_H$.  
%implying the existence of two trends: a weakly absorbed and soft case with $N_H \sim 10^{21}\ \mathrm{cm^{-2}}$ and $\Gamma \sim 5$ and a heavily absorbed and hard case with $N_H \sim 10^{23}\ \mathrm{cm^{-2}}$ and $\Gamma \sim 1$.
We also confirm yearly and monthly variabilities of flux for some \hsS.
We propose that \rxj\ is embedded in a complex surroundings where some dense molecular clumps and cores exist inside a wind-blown cavity, and 
that the \hs\ traces synchrotron emission caused by an interaction of shock waves of the SNR and dense molecular cores
with a number density of $10^{5}\--10^{7}~ \mathrm{cm}^{-3}$.
The X-ray radiation of the \hs\ might be emitted from both primary electrons accelerated at the shocks and secondary electrons produced by the interaction of accelerated protons with the cores.


